In-Context Learning for Few-Shot Nested Named Entity Recognition

In nested Named entity recognition (NER), entities are nested with each other, and thus requiring more data annotations to address. This leads to the development of few-shot nested NER, where the prevalence of pretrained language models with in-context learning (ICL) offers promising solutions. In this work, we introduce an effective and innovative ICL framework for the setting of few-shot nested NER. We improve the ICL prompt by devising a novel example demonstration selection mechanism, EnDe retriever. In EnDe retriever, we employ contrastive learning to perform three types of representation learning, in terms of semantic similarity, boundary similarity, and label similarity, to generate high-quality demonstration examples. Extensive experiments over three nested NER and four flat NER datasets demonstrate the efficacy of our system.

==> refs-bak.tex <==
@inproceedings{zhang-etal-2019-openki,
    title = "{O}pen{KI}: {I}ntegrating {O}pen {I}nformation {E}xtraction and {K}nowledge {B}ases with {R}elation {I}nference",
    author = "Zhang, Dongxu  and
      Mukherjee, Subhabrata  and
      Lockard, Colin  and
      Dong, Luna  and
      McCallum, Andrew",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    year = "2019",
    pages = "762--772",
}
@article{ZhangZYL21,
  author       = {Mengli Zhang and
                  Gang Zhou and
                  Wanting Yu and
                  Wenfen Liu},
  title        = {{FAR-ASS:} Fact-aware reinforced abstractive sentence summarization},
  journal      = {Inf. Process. Manag.},
  volume       = {58},
  number       = {3},
  pages        = {102478},
  year         = {2021},
}
@inproceedings{LuPRAWW19,
  author       = {Xiaolu Lu and
                  Soumajit Pramanik and
                  Rishiraj Saha Roy and
                  Abdalghani Abujabal and
                  Yafang Wang and
                  Gerhard Weikum},
  title        = {Answering Complex Questions by Joining Multi-Document Evidence with
                  Quasi Knowledge Graphs},
  booktitle    = {Proceedings of the 42nd International {ACM} {SIGIR} Conference on
                  Research and Development in Information Retrieval},
  pages        = {105--114},
  year         = {2019},
}
@inproceedings{yates-etal-2007-textrunner,
    title = "{T}ext{R}unner: Open Information Extraction on the Web",
    author = "Yates, Alexander  and
      Banko, Michele  and
      Broadhead, Matthew  and
      Cafarella, Michael  and
      Etzioni, Oren  and
      Soderland, Stephen",
    booktitle = "Proceedings of Human Language Technologies: The Annual Conference of the North {A}merican Chapter of the Association for Computational Linguistics ({NAACL}-{HLT})",
    year = "2007",
    pages = "25--26",
}

@inproceedings{0001WLLLQZZC22,
  author       = {Hao Fei and
                  Shengqiong Wu and
                  Jingye Li and
                  Bobo Li and
                  Fei Li and
                  Libo Qin and
                  Meishan Zhang and
                  Min Zhang and
                  Tat{-}Seng Chua},
  title        = {LasUIE: Unifying Information Extraction with Latent Adaptive Structure-aware
                  Generative Language Model},
  booktitle    = {Proceedings of Advances in Neural Information Processing Systems, NeurIPS},
  year         = {2022},
}

@inproceedings{gomez-rodriguez-etal-2018-global,
    title = "Global Transition-based Non-projective Dependency Parsing",
    author = "G{\'o}mez-Rodr{\'\i}guez, Carlos  and
      Shi, Tianze  and
      Lee, Lillian",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    year = "2018",
    pages = "2664--2675",
}

@inproceedings{kitaev-klein-2018-constituency,
    title = "Constituency Parsing with a Self-Attentive Encoder",
    author = "Kitaev, Nikita  and
      Klein, Dan",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    year = "2018",
    pages = "2676--2686",
}
@inproceedings{fei-etal-2021-better,
    title = "Better Combine Them Together! Integrating Syntactic Constituency and Dependency Representations for Semantic Role Labeling",
    author = "Fei, Hao  and
      Wu, Shengqiong  and
      Ren, Yafeng  and
      Li, Fei  and
      Ji, Donghong",
    booktitle = "Findings of the Association for Computational Linguistics: ACL-IJCNLP 2021",
    year = "2021",
    pages = "549--559",
}

@inproceedings{li2022unified,
  title={Unified named entity recognition as word-word relation classification},
  author={Li, Jingye and Fei, Hao and Liu, Jiang and Wu, Shengqiong and Zhang, Meishan and Teng, Chong and Ji, Donghong and Li, Fei},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={10965--10973},
  year={2022}
}

@inproceedings{huang-chiang-2005-better,
    title = "Better k-best Parsing",
    author = "Huang, Liang  and
      Chiang, David",
    booktitle = "Proceedings of the Ninth International Workshop on Parsing Technology",
    year = "2005",
    pages = "53--64",
}
@inproceedings{wei-etal-2019-imitation,
    title = "Imitation Learning for Non-Autoregressive Neural Machine Translation",
    author = "Wei, Bingzhen  and
      Wang, Mingxuan  and
      Zhou, Hao  and
      Lin, Junyang  and
      Sun, Xu",
    booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
    year = "2019",
    pages = "1304--1312",
}
@inproceedings{song-etal-2019-leveraging,
    title = "Leveraging Dependency Forest for Neural Medical Relation Extraction",
    author = "Song, Linfeng  and
      Zhang, Yue  and
      Gildea, Daniel  and
      Yu, Mo  and
      Wang, Zhiguo  and
      Su, Jinsong",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    year = "2019",
    pages = "208--218",
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
}

@inproceedings{lewis-etal-2020-bart,
    title = "{BART}: Denoising Sequence-to-Sequence Pre-training for Natural Language Generation, Translation, and Comprehension",
    author = "Lewis, Mike  and
      Liu, Yinhan  and
      Goyal, Naman  and
      Ghazvininejad, Marjan  and
      Mohamed, Abdelrahman  and
      Levy, Omer  and
      Stoyanov, Veselin  and
      Zettlemoyer, Luke",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    year = "2020",
    pages = "7871--7880",
}

@article{RaffelSRLNMZLL20,
  author  = {Colin Raffel and Noam Shazeer and Adam Roberts and Katherine Lee and Sharan Narang and Michael Matena and Yanqi Zhou and Wei Li and Peter J. Liu},
  title   = {Exploring the Limits of Transfer Learning with a Unified Text-to-Text Transformer},
  journal = {Journal of Machine Learning Research},
  year    = {2020},
  volume  = {21},
  number  = {140},
  pages   = {1--67},
}


@inproceedings{VelickovicCCRLB18,
  author    = {Petar Velickovic and
               Guillem Cucurull and
               Arantxa Casanova and
               Adriana Romero and
               Pietro Li{\`{o}} and
               Yoshua Bengio},
  title     = {Graph Attention Networks},
  booktitle = {Proceedings of the 6th International Conference on Learning Representations, {ICLR}},
  pages={35--45},
  year      = {2018},
}


@inproceedings{VinyalsFJ15,
  author    = {Oriol Vinyals and
               Meire Fortunato and
               Navdeep Jaitly},
  title     = {Pointer Networks},
    booktitle = {Proceedings of the International Conference on Neural Information Processing},
  pages     = {2692--2700},
  year      = {2015},
}




@inproceedings{chopra2005learning,
  title={Learning a similarity metric discriminatively, with application to face verification},
  author={Chopra, Sumit and Hadsell, Raia and LeCun, Yann},
  booktitle={Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR)},
  volume={1},
  pages={539--546},
  year={2005},
}

@inproceedings{cui-etal-2018-neural,
    title = "Neural Open Information Extraction",
    author = "Cui, Lei  and
      Wei, Furu  and
      Zhou, Ming",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)",
    year = "2018",
    pages = "407--413",
}

@inproceedings{kolluru-etal-2020-imojie,
    title = "{IM}o{JIE}: Iterative Memory-Based Joint Open Information Extraction",
    author = "Kolluru, Keshav  and
      Aggarwal, Samarth  and
      Rathore, Vipul  and
      {Mausam}  and
      Chakrabarti, Soumen",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    year = "2020",
    pages = "5871--5886",
}
@inproceedings{kolluru-etal-2020-openie6,
    title = "{O}pen{IE}6: {I}terative {G}rid {L}abeling and {C}oordination {A}nalysis for {O}pen {I}nformation {E}xtraction",
    author = "Kolluru, Keshav  and
      Adlakha, Vaibhav  and
      Aggarwal, Samarth  and
      {Mausam}  and
      Chakrabarti, Soumen",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    year = "2020",
    pages = "3748--3761",
}
@inproceedings{ZhanZ20,
  author       = {Junlang Zhan and
                  Hai Zhao},
  title        = {Span Model for Open Information Extraction on Accurate Corpus},
  booktitle    = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
                  2020, The Thirty-Second Innovative Applications of Artificial Intelligence
                  Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
                  Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
                  February 7-12, 2020},
  pages        = {9523--9530},
  year         = {2020},
}

@article{abs-2009-08128,
  author       = {Youngbin Ro and
                  Yukyung Lee and
                  Pilsung Kang},
  title        = {Multi{\^{}}2OIE: Multilingual Open Information Extraction based on
                  Multi-Head Attention with {BERT}},
  journal      = {CoRR},
  volume       = {abs/2009.08128},
  year         = {2020},
}

@inproceedings{solawetz-larson-2021-lsoie,
    title = "{LSOIE}: A Large-Scale Dataset for Supervised Open Information Extraction",
    author = "Solawetz, Jacob  and
      Larson, Stefan",
    booktitle = "Proceedings of the 16th Conference of the European Chapter of the Association for Computational Linguistics: Main Volume",
    year = "2021",
    pages = "2595--2600",
}
@inproceedings{dong-etal-2022-syntactic,
    title = "Syntactic Multi-view Learning for Open Information Extraction",
    author = "Dong, Kuicai  and
      Sun, Aixin  and
      Kim, Jung-Jae  and
      Li, Xiaoli",
    booktitle = "Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing",
    year = "2022",
    pages = "4072--4083",
}
@article{abs-2305-03299,
  author       = {Kuicai Dong and
                  Aixin Sun and
                  Jung{-}Jae Kim and
                  Xiaoli Li},
  title        = {Open Information Extraction via Chunks},
  journal      = {CoRR},
  volume       = {abs/2305.03299},
  year         = {2023},
}

@inproceedings{stanovsky-dagan-2016-creating,
    title = "Creating a Large Benchmark for Open Information Extraction",
    author = "Stanovsky, Gabriel  and
      Dagan, Ido",
    booktitle = "Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing",
    year = "2016",
    pages = "2300--2305",
}

@inproceedings{gashteovski-etal-2022-benchie,
    title = "{B}ench{IE}: A Framework for Multi-Faceted Fact-Based Open Information Extraction Evaluation",
    author = "Gashteovski, Kiril  and
      Yu, Mingying  and
      Kotnis, Bhushan  and
      Lawrence, Carolin  and
      Niepert, Mathias  and
      Glava{\v{s}}, Goran",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    year = "2022",
    pages = "4472--4490",
}
@inproceedings{bhardwaj-etal-2019-carb,
    title = "{C}a{RB}: A Crowdsourced Benchmark for Open {IE}",
    author = "Bhardwaj, Sangnie  and
      Aggarwal, Samarth  and
      Mausam, Mausam",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    year = "2019",
    pages = "6262--6267",
}

@inproceedings{lechelle-etal-2019-wire57,
    title = "{W}i{R}e57 : A Fine-Grained Benchmark for Open Information Extraction",
    author = "Lechelle, William  and
      Gotti, Fabrizio  and
      Langlais, Phillippe",
    booktitle = "Proceedings of the 13th Linguistic Annotation Workshop",
    year = "2019",
    pages = "6--15",
}




% LM
@inproceedings{devlin-etal-2019-bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
      booktitle = {Proceedings of the North American Chapter of the Association for Computational Linguistics},
    year = "2019",
    pages = "4171--4186",
}


@inproceedings{PetersNIGCLZ18,
  author    = {Matthew E. Peters and
               Mark Neumann and
               Mohit Iyyer and
               Matt Gardner and
               Christopher Clark and
               Kenton Lee and
               Luke Zettlemoyer},
  title     = {Deep Contextualized Word Representations},
      booktitle = {Proceedings of the North American Chapter of the Association for Computational Linguistics},
  pages     = {2227--2237},
  year      = {2018}
}



